Vector Quantized Models for Planning

Recent developments in the field of model-based RL have proven successful in a range of environments, especially ones where planning is essential. However, such successes have been limited to deterministic fully-observed environments. We present a new approach that handles stochastic and partially-observable environments. Our key insight is to use discrete autoencoders to capture the multiple possible effects of an action in a stochastic environment. We use a stochastic variant of Monte Carlo tree search to plan over both the agent's actions and the discrete latent variables representing the environment's response. Our approach significantly outperforms an offline version of MuZero on a stochastic interpretation of chess where the opponent is considered part of the environment. We also show that our approach scales to DeepMind Lab, a first-person 3D environment with large visual observations and partial observability.

==> acknowledgements.tex <==
\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.


==> old/introduction-old.tex <==
\section{Introduction}

%Abilities to learn about the world and make predictions are regarded as key ingredients of truly intelligent agents. Humans are known to build models of the world which allow us to devise and enact plans to reach our goals. 
% In artificial intelligence research, planning with models have reached state-of-the-art performance in games like chess \citep{alphazero}, Go \citep{alphago, alphagozero}, and Poker \citep{moravvcik2017deepstack, brown2017libratus}. However, such methods rely on access to a simulator for self-play or for lookahead search. Recently proposed approaches like \emph{MuZero} \citep{schrittwieser2019mastering} learn models for lookahead search but these models are deterministic, limiting the viability of such approaches to deterministic environments and full information \emph{and} deterministic games. Further it also requires knowledge of the nature of the game being played, such as the number of players in the game and their action spaces. In the general multi-agent reinforcement learning setting, stochasticity could arise from the transition dynamics of the environment, from the stochastic policies of other agents, or from the agent's lack of complete knowledge about the state of the environment and other agents.
%Ideally, an intelligent agent should be able to occupy a shared world with unknown number of other agents of various types and learn from experience without making a priori assumptions about the world.
%Thus, in this work, we introduce a model-based reinforcement learning approach wherein we learn stochastic models purely from the agent's observations and actions. Further, stochasticity from multiple sources is distilled into \emph{controllable} discrete latent variables \citep{oord2017neural}. This allows using planning algorithms like \emph{Monte Carlo tree search} \citep{coulom2006efficient} (which are typically only applicable to deterministic full information games) by effectively considering these discrete latent variables as "actions" outside of the agent itself. 
%The only strong assumption made by our model is knowledge of the observation and action space for the agent being trained.

Learning predictive models about the world is regarded as key ingredient of truly intelligent agents. Humans are known to build models of the world which allow us to devise and enact plans to reach our goals. In artificial intelligence research, planning with models have reached state-of-the-art performance in games like chess \citep{alphazero}, Go \citep{alphago, alphagozero}, and Poker \citep{moravvcik2017deepstack, brown2017libratus}. However, such methods typically only feasible for games with known rules since they rely on access to a simulator for self-play or for lookahead search. Recently proposed approaches like \emph{MuZero} \citep{schrittwieser2019mastering} learn models for lookahead search which relax the requirement for knowing the rules of the game. However, these models are deterministic, thus, limiting the viability of such approaches to deterministic environments and full information \emph{and} deterministic games. Further more, in MuZero, MCTS branches its decision on the order of players and action space tied to the environment, which means they still need to know the nature of the game being played. While they are making efficient use of the model by exploiting the symmetry in two player games, it is not general enough for many real world problem. 

In the general multi-agent reinforcement learning setting, stochasticity could arise from the transition dynamics of the environment, from the stochastic policies of other agents, or from the agent's lack of complete knowledge about the state of the environment and other agents. Ideally, an intelligent agent should be able to occupy a shared world with unknown number of other agents of various types and learn from experience without making a priori assumptions about the world.

\sherjil{Specifically explain problem with current methods, and explain how we solve it.}

In this work, we address the issue of stochasticity and extend the success of MCTS to general environments with partial observability and unknown rules. Our contributions are as follows:

\begin{itemize}
    \item We propose a discrete latent variable world model that captures stochasticity of the environment;
    \item We distill these latent variables into \emph{controllable} variables which we could think them as "actions" outside of the agent itself;
    \item We unlock planning over learned environment dynamics via these \emph{controllable} discrete latent variables disentangled from the action space tied to environment both in branching and in time.
\end{itemize}

% This requires learning models which can handle partial observability, environment stochasticity, and learning only from the agent's observations and actions, i.e. the general reinforcement learning setting.
% In this work we propose a technique to learn discrete stochastic world models which handle environment and opponent stochasticity and handles partial observability.

% The ability and make predictions about the world is regarded as a key ingredient of intelligent agents \citep{clark2013whatever}. A long-standing objective in artificial intelligence has been to incorporate use of predictions in agents to make intelligent decisions \citep{lake2017building}. However, the high-dimensional nature of real-world sensory data makes it challenging to learn predictive models. A number of deep neural network-based generative models have been introduced for images, text, audio, and video. Likelihood-based generative models \citep{van2016conditional,kingma2013auto} are designed to model all modes of a distribution, and thus are suitable for learning predictive models since an agent needs to have an accurate understanding of all possible consequences of its actions. However, likelihood-based deep generative models are known to underperform in terms of sample quality compared to implicit generative models such as generative adversarial networks (GANs) \citep{goodfellow2014generative}. GANs learn a stochastic generator which is able to choose parts of the data distribution to synthesize. While they are able to synthesize high-fidelity images \citep{brock2018large} and audio \citep{binkowski2019high}, they are known to drop large parts of the data distribution \citep{bau2019seeing}, and thus are unsuitable for learning forward models for planning \textcolor{red}{since good planning requires taking into account all contingencies}.

% \cite{kawato2003internal}: evidence brain learns internal models.

% More recently, \emph{partial} models \cite{gregor2019shaping,rezende2020causally} have been introduced.

% Three ways to do MBRL. All three have issues.

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/figure.png}
    \caption{TODO: 
    \begin{enumerate}
    \item Show value/reward predictions.
    \item Show visit counts. 
    \item Show best selected line, and best action. 
    \item Show training graph.
    \end{enumerate}
    }
    \label{fig:summary_figure}
    
\end{figure}

% <Human beings have multiple modalities of high-dimensional sensory information>.

% \textcolor{red}{
% \begin{enumerate}
%     \item We know from neuroscience that brains operate by making predictions about the world and using to act \cite{clark2013whatever}.
%     \item Inspired by such research from neuroscience, a popular thread in model-based reinforcement learning research is to use agent experience to learn a model of the world which is then combined with planning algorithms to act on the world to optimize rewards or reach goals.
%     \item Learning such world models for complex environments is a challenging problem though. For environments which have large images as observations, this requires generative modeling of images, which is a challenging problem [image generative models citations]. Discuss likelihood-based models vs GANs.
%     \item Because of these complexities, an alternative to do learn partial models. They have been successful as well \cite{schrittwieser2019mastering}, but recent work identifies that partial models can be causally incorrect [Rezende et al.]. The authors propose using backdoor, however the ideal backdoor is either the full observation or requires access to the optimal policy.
%     \item Recently, we've made an advance in likelihood-based generative modeling. Introduce VQ-VAE.
%     \item We extend VQ-VAE to the temporal domain.
% \end{enumerate}
% }

% TODO
% Introduce 
